TBSSvis: Visual Analytics for Temporal Blind Source Separation

Temporal Blind Source Separation (TBSS) is used to obtain the true underlying processes from noisy temporal multivariate data, such as electrocardiograms. TBSS has similarities to Principal Component Analysis (PCA) as it separates the input data into univariate components and is applicable to suitable datasets from various domains, such as medicine, finance, or civil engineering. Despite TBSS's broad applicability, the involved tasks are not well supported in current tools, which offer only text-based interactions and single static images. Analysts are limited in analyzing and comparing obtained results, which consist of diverse data such as matrices and sets of time series. Additionally, parameter settings have a big impact on separation performance, but as a consequence of improper tooling, analysts currently do not consider the whole parameter space. We propose to solve these problems by applying visual analytics (VA) principles. Our primary contribution is a design study for TBSS, which so far has not been explored by the visualization community. We developed a task abstraction and visualization design in a user-centered design process. Task-specific assembling of well-established visualization techniques and algorithms to gain insights in the TBSS processes is our secondary contribution. We present TBSSvis, an interactive web-based VA prototype, which we evaluated extensively in two interviews with five TBSS experts. Feedback and observations from these interviews show that TBSSvis supports the actual workflow and combination of interactive visualizations that facilitate the tasks involved in analyzing TBSS results.

==> sections/04-visualization.tex <==
\section{Visualization Design \& Justification}
\label{sec:app}

In this section, we present the visualization design we obtained based on the task abstraction (\Fref{sec:task-abstraction}) and implemented in a web-based prototype for gSOBI. A design goal is to make \toolname{} generic enough to allow its use in many application domains, because, like PCA, TBSS is a domain-independent method (cf. \Fref{sec:conclusion--transferability}). We designed \toolname{} for inputs with the length of up to 5\,000 time steps, and up to 50 dimensions. While these limits do not accommodate extreme cases, like fMRI data (100+ dimensions, 100\,000+ time steps), we expect it is enough for many applications. The dataset we used for images is the financial dataset from \Fref{sec:datasets--exrates}. 
%Using RStudio, the analyst's current tool, the same analysis possible in \toolname{} would involve a) programming several static visualizations manually, b) searching for them in the history of generated plots, because they can only be viewed one at a time and c) manually programming some analysis techniques.

% the usage scenario should less be "list of things you can do" and more "here's how toolname changes the analysis process"
% angles in which tbssvis is better:
% - interactions and visualizations designed for the tasks make common things faster
% - guidance for parameter selection makes them consider a larger parameter space, as by common assumption they investigate only a small fraction (first m lags) - but tbssvis often confirmed that this fraction is not bad
% - other automated analyses, such as the clustering, answer questions they previously had no answer
\begin{figure}
  \centering
  \includegraphics[width=\textwidth]{images/app/usage-scenario-exrates.png}
  \caption{Usage scenario with \toolname{} on a dataset of currency exchange rates. Temporal order of visualizations is indicated by a thick curved gray line. (A) shows input data, (B–G, I) show similarity of members on different levels and aspects, (H–J) are used to select parameters. Visualizations are distributed across three screens \emph{Data Load} (\Fref{sec:app--data-load}, A), \emph{Explore} (\Fref{sec:app--explore}, B–G and K) and \emph{Parameter Selection} (\Fref{sec:app--parameter-selection}, H–J).}
  \label{fig:app--usage-scenario}
\end{figure}

%A
%First, the analyst opens \toolname{} with the dataset already loaded. At first they see the input data in the \textit{Data Load} screen (\Fref{sec:app--data-load}). Using their current tools, it would already be difficult to see so much data simultaneously as R by default displays only 10~time series. There is a large spike in the last input variable so they zoom in interactively, which is not possible in RStudio, to investigate if it is an error in the data (\Fref{fig:app--usage-scenario}A). After this, they continue to the \textit{Explore} screen (\Fref{sec:app--explore}).

%B
%Here, they first look at the similarity projection of the precomputed ensemble (\Fref{fig:app--usage-scenario}B, \Fref{sec:app--explore--projections}) to determine the overall similarity structure according to obtained components. While the analyst can assess the similarity of two members in RStudio, these views allow them to compare many more simultaneously. As the left three points seem rather close, the analyst selects the outlier (red) and the most central of the other members (blue) for more detailed inspection. Data related to these members are highlighted with the assigned color hues in all views of this screen.

%C
%The analyst looks at the table (\Fref{fig:app--usage-scenario}C, \Fref{sec:app--explore--table}) to see if their parameters are any different, and what parameters lead to a successful result. It is visible that the blue member predominantly uses one lag set, while the red has a more equally distributed setting.

%D
%In the parameter comparison view (\Fref{fig:app--usage-scenario}D, \Fref{sec:app--explore--parameter-comparison}) the same data are displayed in more detail. The analyst learns that the blue member used more and very short lags, unlike the red member. No default visualizations for most of the analyst's tasks exist in their current tool.

%E
%The analyst takes a look at the component overview (\Fref{fig:app--usage-scenario}E, \Fref{sec:app--explore--component-overview}) to investigate the similarity of the red and blue members to each other but also to the rest of the ensemble. After adjusting the clustering parameter, the analyst learns that the first three components are more similar to each other than to other components in the sets, the eight and ninth are contained only in the blue member and the sixth is in neither. To assess the overall stability of components, they can unselect the red and blue member and look for mostly black bars in the histograms.

%F
%The analyst now wants to compare the first components of the red and blue member in detail. To do so, they open the component comparison view (\Fref{fig:app--usage-scenario}F, \Fref{sec:app--explore--slope}), superimpose the two component sets and enlarge the Y axis of the first graph. It becomes apparent that the two components are mostly noise, with values around zero, and that they are not at all similar apart from the spike. The large bar on the left of the line graph confirms this.

%G, H, I
%The analyst now wants to try a new parameter setting and see how it compares to red and blue. They open the \textit{Parameter Selection} (\Fref{sec:app--parameter-selection}) screen, pick a higher weight than either red or blue (\Fref{fig:app--usage-scenario}G), and proceed to the lag selection (\Fref{fig:app--lag-selection}, \Fref{sec:app--parameter-selection--lag-selection}). The analyst expects underlying processes of power consumption data to exhibit high weekly correlation and thus adjusts the lags to weekly resolution. Looking for the most promising lags, they filter for a high eigenvalue measure (\Fref{fig:app--usage-scenario}H). It becomes apparent in the multivariate autocorrelation function plot (\Fref{fig:app--usage-scenario}I) that larger lags, where input variables correlate negatively, should also be considered. This is something the analyst likely would have missed using their current tools, because programming such an analysis is laborious and requires time they usually do not have. The analyst interactively selects $\boldsymbol k_1$ lags based on the guidance by \toolname{}, accepts the defaults for $\boldsymbol k_2$ and is then redirected back to the \textit{Explore} screen. The new ensemble member is automatically selected once available and is assigned the next possible color, in this case green.

% J
%The analyst again opens the component comparison view (\Fref{fig:app--usage-scenario}J, \Fref{sec:app--explore--slope}) to inspect the components of selected members in detail. They adjust the plotting order to red-green-blue to compare the green member to both red and blue simultaneously. They see that their custom parameter setting yielded yet another quite dissimilar result, as only a few components exist in all three members.

% K
%To learn how these components were formed by the input data, the analyst opens the matrix comparison view (\Fref{fig:app--usage-scenario}K, \Fref{sec:app--explore--matrix}). The small heatmap (bottom left) shows again that the three members are quite dissimilar. From the matrix visualizations it becomes apparent that components of the green member are easier to interpret than those from the other members, because there is mostly one large factor per component.

% the rest
% can they confirm good parameter settings? i guess they can if e.g. a result doesn't change to an existing, then the lags used there didn't carry much information
%From here on the analyst continues in this loop and interactively compares components, forms hypotheses about suitable parameter settings, confirms them visually and numerically based on how dissimilar a new member is in terms of components obtained and parameters used, and reasons about what the best result could be. With one click it is possible to export candidates for the latter to a file format supported by their current tool, where the data processing pipeline continues.
\subsection{Data Load}
\label{sec:app--data-load}

% WHY
% analysis goal
% see input data
% low level tasks involved
% identify input data (same as components)
% WHAT
% input data
% HOW
% line graphs

% what analyst wants to do
%First of all, our analyst wants to see the raw input data, mostly to verify their correctness but also to explore interesting features in the input data. Using their current tools, this involves plotting static line graphs in full detail into a very constrained space, thereby often rendering any features invisible.

% how it works
The first view of \toolname{} shows raw input data, where all input time series are plotted vertically aligned and ordered by variable name. The display of and interaction with all time series in \toolname{} is handled by the same logic as shown in \Fref{fig:time-series-anatomy}. Due to the length and amount of time series, we employ semantic zooming and at first save display space by drastically reducing their Y axis and omitting any labels by default. This can be changed with interaction: On hover, we display axis labels for the hovered time series, and the Y axis can be increased individually. If an analyst is interested in a contiguous subset of the time series, it is possible to zoom in with brushing, which will affect all time series in the application. Both the semantic and temporal zoom can be reset with interactions recommended by Schwab et al. \cite{schwab2019}.

\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{images/app/time-series-anatomy.png}
  \caption{Display of and interaction with time series. (A) A time series is displayed with a line graph, an optional label, and an optional bar to its left. The bar encodes a DOI function of a time series. (B) Typical vertical arrangement of multiple time series in \toolname{}. The user enlarged the first and last time series and hovered over the third, thus its X axis labels are shown.}
  \label{fig:time-series-anatomy}
\end{figure}

% an insight from the study
%Looking at \toolname{}'s visualizations (\Fref{fig:app--usage-scenario}A), the analyst is quickly able to identify, e.g., the Great Recession of 2007–2009, as it is marked by more volatile time spans with large spikes. Not knowing what to expect, the analyst wants to see possible TBSS results and try their own parameter settings.

% the lag boundary has been a footnote since forever, we don't talk about it. if we did, this would be the paragraph:

% In the right half, the analyst can reduce the default lag boundary. Every lag-based visualization and computation ends at the configured lag boundary, which by default is the largest lag that contains at least 25 \% of all time steps. This saves computation time and display space, and reducing the lag boundary is useful e.g. when one considers high-frequency input time series, such as EEG data, where at the same time the temporal correlation is believed to be short. The lag boundary is changed by selecting a shorter lag using the lag selection component (\autoref{sec:app--parameter-selection--lag-selection}). The proceed button navigates to the ``Explore'' screen.

\subsection{Explore}
\label{sec:app--explore}

% what does the analyst want
The \textit{Explore} screen (\Fref{fig:app--explore}) allows analysts to explore, browse, and compare ensemble members and select them for detailed comparison according to their parameters, components, and other data. It can follow immediately to \textit{Data Load} without user-provided parameters because we compute five settings automatically: The defaults of gSOBI's R package, a recommendation from the literature \cite{tang2005a}, and three random settings. %Let us assume for now that the analyst is interested in the differences of the precomputed results, before they try custom parameter settings.

% LHS \cite{stein1987}.

\begin{figure}
  \centering
  \includegraphics[width=\textwidth]{images/app/explore-exrates.png}
  \caption{The Explore view. It shows ensemble members with their parameter settings (A), similarity projections of the ensemble regarding parameters and components (B), an overview of components found in all ensemble members (C), and a section for more detailed comparisons (D), currently displaying the scatter diagonality (\Fref{sec:app--explore--diagonality}). Data pertaining to a selected member is encoded with its assigned color hue in all views.}
  \label{fig:app--explore}
\end{figure}

% how does it work
The \textit{Explore} screen is divided into four linked views, which correspond to tasks in \Fref{sec:task-abstraction--tasks}, and a toolbar on top:

\begin{itemize}
  \item[A] A table representation of ensemble members (one member represents one run) with summaries of parameters and the outcome (Task I1, \Fref{fig:app--explore}A). The analyst can compare parameter settings of different runs at a glance.
  \item[B] Similarity projections of components and lag sets (Tasks C2, C4, \Fref{fig:app--explore}B). They allow to quickly assess the relative similarities of different runs with regard to obtained components and used parameters.
  \item[C] An overview of obtained components in all members (Task C4, \Fref{fig:app--explore}C). Using that, analysts can quickly find stable and unstable components. 
  \item[D] A detail area where selected members can be inspected and compared in multiple tabs dependent on the task at hand (Tasks I1–I4 and C1–C5, \Fref{fig:app--explore}D).
\end{itemize}

The visual arrangement is from left to right, and from overview (visual summaries) to detail (comparison views). Individual sections can be collapsed by clicking the vertical text on its left top, to support smaller screens.

% how does it work
% use of color
It is necessary to discuss how color is used in this screen. According to Mackinlay \cite{mackinlay1986}, color is the most effective visual variable for nominal data after position, and, therefore, often used to encode different data classes. In multiple views, the same classes should be encoded with the same palette \cite{qu2018}. Because humans can only reasonably distinguish a few different colors, we cannot statically assign colors to all ensemble members. We, therefore, use a user-controlled dynamic assignment of colors of a qualitative palette from ColorBrewer2 \cite{brewer2013}. The available colors are displayed in the toolbar and can be reordered with drag \& drop. When hovering over an unselected member, the next free color (left to right) is a) used to highlight its related data in all views and b) associated to the member when selected. As one color is always needed for highlighting, the last free color cannot be used for selection. The color order determines the plotting order in all comparison views.

% use of sorting
% this is important when we compute multidimensional distances which usually involves vectors
Another cross-cutting concern is the ordering of components. As described in \Fref{sec:task-abstraction}, the order of components is not defined. In practice, this means that analysts use measures which are sign-independent to compare components, such as absolute Pearson correlation, and impose an order by sorting components according to a function. We will call this a \textit{degree-of-interestingness function} (DOI), and require it to be any function $f: \mathbb{R}^n \rightarrow \mathbb{R}$ that maps a time series of length $n$ to a single number. Because TBSS is a domain-independent method, many DOI functions could be useful \cite{fu2011} depending on what the domain's interesting features are. Based on discussions with our collaborators we use the absolute third (skewness) and fourth (kurtosis) moment in \toolname{}. These are useful to find the most skewed components and those with the most outlying values, as the first two moments (mean and variation) of all components are identical. The DOI function can be changed in the toolbar, and all views that show component-related data will update as the set members are sorted in descending order based on the new DOI function values.

\subsubsection{Table (Task I1)}
\label{sec:app--explore--table}

% WHY
% analysis goal
% see what parameters were used so far
% low level tasks involved
% identify parameters
% WHAT
% parameters
% HOW
% bar charts

% what analyst wants
%The analyst, knowing that some runs were precomputed, now wants to see which parameter settings were used. Using their current tools, this means looking at a lot of numbers, if analysts even made an effort to save past settings, as no tooling or conventions to visualize this data exist.

% how it works
We use a table as it is a simple way to present visual summaries. Column names are based on the R API of gSOBI (compare \Fref{fig:app--explore}A). The \textit{Method} is a unique and deterministic identifier for a run, to distinguish it from others with very similar parameters. The background of the cell encodes the success status. The \textit{b} column shows the weight parameter on a vertically aligned scale.
%, so it can easily be compared between rows. The axis is aligned such that the triangle mark is next to the lag set which would exclusively be used on either end, and we use a power scale to enlarge the value range analysts are most interested in. 
As a visual summary of a lag set, we show a small histogram of the used lags (\textit{k1}, \textit{k2}).
%The bin size is chosen automatically such that the histogram shows six bins. 
It is the same visualization as in the comparison view (\Fref{sec:app--explore--parameter-comparison}). Here, bar length encodes maximum value per row, to support Task I1.
The last column contains controls for two actions, encoded with icons. The left icon will navigate to the parameter selection screen, with the run's parameters already selected. This way we support a ``what if'' parameter analysis, in which analysts can easily vary a single parameter and compare the outcome. The right icon is used to download involved data as .RData, which is supported by our users' current tool. There, they can continue analysis with more customized or domain-specific tools if necessary.

% insight from the study
%The analyst can easily assess the overall variance in parameters (\Fref{fig:app--usage-scenario}B) and decide which setting they would like to add. More insights are possible in connection with the similarity projections.

\subsubsection{Similarity Projections (Tasks C2, C4)}
\label{sec:app--explore--projections}

% WHY
% analysis goal
% see similar results
% low level tasks involved
% compare component sets
% WHAT
% component sets
% HOW
% dimension reduction

% what analyst wants
%After getting an overview of the used parameter settings, the analyst wants to know how the runs compare in terms of obtained components. Currently, analysts plot components side by side and look for differences. Obviously, this only works for very few components and sets, but already at this point there are in total 92~components to consider.

We facilitate their analysis by relating all component sets and parameters in terms of similarity/dissimilarity. A 2D-embedding, where similar position encodes similarity in another space, seems appropriate from a visualization perspective (see \Fref{fig:app--explore}B). Many options to obtain such an embedding exist, but for our task Multidimensional Scaling (MDS) is suited best as the analyst looks for global clusters \cite{nonato2019}. The input to MDS is a dissimilarity matrix $D$. While $D$ is fixed for lag set similarity projections (Manhattan distance of the lag set histograms), we allow the user to choose from different dissimilarity functions to build $D$ for the component similarity projection, to work with either single components or the set, and either on correlation or DOI as dissimilarity. The dissimilarity we will use in other views as well is $dist_{cor}(c_i, c_j) = 1 - | cor(c_i, c_j) |$, where $cor$ is the Pearson correlation. The absolute value accounts for the ambiguous sign of components.

As MDS will project elements with same values in high-dimensional space to the same low-dimensional points, we would soon run into an occlusion problem—consider an analyst who keeps lag sets the same, but varies only the weight. There are a couple of ways to deal with occlusion, most notably lenses \cite{tominski2017}. However, our users are not used to complex interactions, so we changed the tradeoff between position accuracy and occlusion. As an implementation of CorrelatedMultiples \cite{liu2018a} was not available, we only rasterize the MDS plot and move overlapping points to the next free cell. When hovering over a point, the other points will change their size proportionally to the original dissimilarity, thereby allowing analysts to investigate projection errors.

%The analyst uses these projections to find parameters settings of similar results. They select two neighboring points in the component similarity projection, then look up their highlighted visual summary of parameters in the table (\Fref{sec:app--explore--table}). The analyst learns that two very different settings (each used only one part of gSOBI exclusively) produced practically identical results, which is something they would not have expected. The analyst selects three results for more detailed analysis (see \Fref{fig:app--usage-scenario}C).

\subsubsection{Component Overview (Task C4)}
\label{sec:app--explore--component-overview}

%After checking the different parameter settings and identifying similar/dissimilar results, the analysts are interested in actual obtained components. They want to see the components themselves but also know how stable they are, e.g., in how many of the results they are found. In their current tool this type of analysis would entail programming custom data mining techniques as this task cannot be solved just visually with almost a hundred components.

We support this analysis by means of a custom clustering scheme. Since it does not make sense here to compare components within-set, but only between-set, we look for a partitioning of all components with the constraint that components of the same set must not be assigned to the same partition. We also want a real representative component of a partition (medoid) for a visual summary. Popular partitioning algorithms such as k-medoids or k-means are not an option here, as they do not work with $dist_{cor}$ (k-means) or do not support the desired constraints (both). To obtain such a constrained k-medoids algorithm, we combined a constrained k-means \cite{wagstaff2001} with a k-means-like version of k-medoids \cite{park2009}. The initial medoids are obtained with FastPAM \cite{schubert2019}, which will in our specific situation already be a good approximation of the final partitioning, as components of the same set have very large dissimilarities. After that, we continue according to \cite{park2009} while also checking the constraints in each iteration, like in \cite{wagstaff2001}.

The component overview (see \Fref{fig:app--explore}C) shows the clustering result. It consists of two parts, a scented widget \cite{willett2007} on top to control the amount of partitions, or clusters, to produce, and a summary of them below. The bar chart of the scented widget shows a clustering quality measure, where high bars indicate a better clustering. Below, we show the medoids of each cluster sorted by the DOI rank of the medoid. To further support Task C4, we show a histogram to the left of the medoid. The histogram shows the rank distribution of the contained components in their respective sets. Additionally, we encode $dist_{cor}$ to the cluster medoid with opacity. This way, stable (stacked bars with high opacity) and unstable (scattered bars with low opacity) components have distinct histogram shapes. Analysts can inspect the actual components by clicking the ``eye'' icon.

% is there an insight? not really, as we don't know the meaning of the components
%Looking at this overview (see \Fref{fig:app--usage-scenario}D), the analyst identifies one component which shows high volatility in 2009. From the rank histogram it is visible that all but the green result agree on this component. The analyst adjusts the clustering parameter to some value with high bars in the scented widget to see if this component is significantly different and moved to its own cluster, which is the case. The analyst decides to compare previously selected results in more detail.

\subsubsection{Parameter Comparison (Task C2)}
\label{sec:app--explore--parameter-comparison}

% what analyst wants
%In previously presented views, the analyst could compare parameters only on a very coarse level (cf. \Fref{fig:app--explore}A). Here, they seek to compare the weight and lag sets in full detail. No default visualizations exist for this analysis in their current tool.

% how it works
To compare weights of different parametrizations, we encode triangle marks on a shared axis (compare \Fref{fig:app--usage-scenario}E). Triangles are stacked in case they otherwise completely occlude each other. To compare lag sets, we use interweaved histograms where the color saturation of a bar encodes the lag size to give an additional visual hint of the lag distribution, and to be consistent with the encoding in the lag selection (\Fref{sec:app--parameter-selection--lag-selection}). First, we compute bins, the size of which is controlled in the toolbar, and frequencies for every lag set. Then, the individual bars are positioned in a grid such that bars of the same lag set are in the same row, and bars representing the same bin are in the same column. To save display space, empty columns are hidden by default, but can be shown after user interaction to revert to the histograms our users are familiar with. Interweaved histograms show distinct images for same (all bars align and have similar height) and different lag sets (bars appear interweaved).

%\begin{figure}
%  \centering
%  \includegraphics[width=\columnwidth]{images/app/histograms.png}
%  \caption{Histograms in tsBSSvis. A: Lag Sets (interweaved). The red and blue lag set both have one lag in bin 1849, whereas the blue lag set has a lag in the bin before, but the red does not. B and C: Ranks of components in different ensembles. B shows agreeing components, C disagreeing.}
%  \label{fig:app--histograms}
%\end{figure}

% insights
%Looking at the interweaved histograms (see \Fref{fig:app--usage-scenario}E), the analyst can see at a glance that the parameters of selected runs do not, in fact, have anything in common. % can i find something more interesting here

\subsubsection{Scatter Diagonality (Task I3)}
\label{sec:app--explore--diagonality}

%As described in the task abstraction the analyst is also interested to compare results on a technical level. In their current tool they would have to program custom data mining techniques, again, which they usually do not have time to.

All data in this view (compare \Fref{fig:app--explore}D) is plotted as a function of the lag, and computed from two types of scatter matrices: The autocovariance matrix, which is what SOBI diagonalizes, and fourth-order cross-cumulant matrices, which are diagonalized by vSOBI. We plot the eigenvalue difference of autocovariance matrices (cf. \Fref{sec:app--parameter-selection}, GO3) to show a measure of temporal structure in the input data.

Underneath, we show how diagonal all possible scatters become by the unmixing matrix of a member. Bars from the lag set histograms (see \Fref{sec:app--explore--parameter-comparison}) are plotted at the top and bottom of the line graph. From that, analysts can form hypotheses about new parametrizations and see how lag selection influenced the scatter diagonality, and choose between competing results. All graphs can be superimposed and zoomed, which will affect all graphs in the tab, similar to how zooming into one time series affects all.

% insights
%While interesting to analysts, this analysis is rarely performed, because it is a lot of work to write the necessary code and visualizations. Therefore, the analyst does not have any expectations here. This might change after repeated analysis on different datasets.

\subsubsection{Unmixing Matrices Comparison (Task C3, I2)}
\label{sec:app--explore--matrix}

%The unmixing matrix holds the linear combination with which the found components can be put back together to the input data. It can be analyzed similar to PCA, where the loadings (factors for each input variable) are of interest. The analyst wants to know which currencies influence the Great Recession component identified in \Fref{sec:app--explore--component-overview}.

We support this task (I2) by showing the factors as a heatmap where a univariate color scale encodes the absolute value in a row with white (low value) to black (\Fref{fig:app--usage-scenario}F). When analysts see interesting patterns, they can select cells, and the respective input data and components will be shown underneath the matrices. This allows to investigate the relationship between inputs and components, and verify if, for example, one input time series is on another scale and then consistently assigned higher factors. In this specific case, analysts can choose to view the factors as if the input data were scaled to unit variance.

Task C3 is also supported, for which we encode the MD-Index \cite{ilmonen2010} of two matrices in a heatmap with a univariate color scale.

%The analyst looked up the number of the component in the component overview (e.g., 8th component of red result) and looks in the according row of the red matrix for non-white cells (see \Fref{fig:app--usage-scenario}F). They learn that it was mainly US dollar, Hong Kong dollar, Thai bhat and Singapore dollar that had an impact. The analyst selects the respective cells and sees that the feature in the component comes mostly from the Thai bhat, although the absolute value of Hong Kong dollar's factor is similar.

\subsubsection{Components Comparison (Task C4)}
\label{sec:app--explore--slope}

%Next, the analyst wants to know which other components of other results are similar to that component, where they are different and if they are maybe even more volatile in the time span 2007–2009. Again also these tasks, in their current tool, entail custom data mining to find similar components from other sets, and custom visualizations to find differences.

In this view, components of each set are color-coded and plotted next to each other in columns (\Fref{fig:app--usage-scenario}). Columns can be reordered by the analyst and rows are sorted by the selected DOI function, therefore allowing flexible comparisons of components and supporting Task C4. The DOI value per set is encoded in the component's bar (see \Fref{fig:time-series-anatomy}).

Analysts can inspect components visually as they are, but they can also display a slope graph between the columns (compare \Fref{fig:app--usage-scenario}G). Lines of the slope graph connect similar components, and thickness encodes similarity from high correlation (thick) to low. This way, it is easy to see stable (thick, single, mostly straight lines) and unstable components (no or thin, multiple, tilted lines), their rank changes and set similarity at a glance. Should analysts suspect that two components are their respective inverse, which is possible in the BSS model, they can change the sign of a component.

%The analyst moves the red result in the middle and looks for incident lines in the 8th component (see \Fref{fig:app--usage-scenario}G). They see that one similar component exists in the blue result and two in the green result.

%To find disagreeing time frames, analysts can superimpose columns, in which case components of same rank in each set will be superimposed, and the time series bar will become gray and show the sum of euclidean distances between all superimposed components. 

\subsection{Parameter Selection}
\label{sec:app--parameter-selection}

To obtain a new result, analysts need to select parameters. They consist in the case of gSOBI of two lag sets and one weight (\Fref{sec:task-abstraction--data}).

To facilitate this selection process, we used the guidance design framework \cite{ceneda2020} to design appropriate guidance \cite{ceneda2017}. Analysts do not know which lags to select and are generally aware of this \emph{knowledge gap}. As discussed in \Fref{sec:task-abstraction--tasks}, the \emph{analysis goal} is to obtain a new/interesting result. Issues occur in the phase of lag selection, because the space of possible lag sets is huge. Analysts currently do not use additional information about lags, mostly due to time constraints. The \emph{knowledge gap} lies in the execution and relates to the input data. We opt for \emph{orienting} guidance, because analysts select lags also based on past experience and domain knowledge, so stronger guidance could be detrimental, and because our guidance \emph{input} is not (cannot be) the ``true'' data: We compute it from the input data, which are per BSS model a linear combination of the components we are interested in. Based on the input data, we calculate guidance \emph{output} per lag that help relate them to each other:

\textit{Guidance Output (GO) 1: Calendar relation.} We compute which lag fits best to intervals in bigger calendar granules. The benefit of this is two-fold. First, lags are abstract and do not consider the calendar used in the data, so thinking in terms of days, weeks, etc., is a more intuitive alternative for someone familiar with the data. Second, it allows us to organize lags by filtering to those which correspond to a difference in a given calendar granule, thereby reducing the amount of lags to reason about. 

\textit{GO2: Largest autocorrelation in input time series.} White noise is a serially uncorrelated process, i.e., does not exhibit autocorrelation, so this measure indicates a latent component might not be white noise.

\textit{GO3: Eigenvalue difference in autocovariance matrices.} The analysts use it to learn more about the input data and it can inform the parameter selection as lags should be chosen such that this eigenvalue difference is big (see \Fref{sec:related-work--tbss}).

\textit{GO4: Scatter diagonality.} This can only be computed when a parametrization of a successful run is refined, i.e., $\hat{\boldsymbol{W}}$ exists. It shows the analyst which selected lags had an impact on the diagonality of autocovariance and fourth cross-cumulant matrices. It can be understood as feedback into the guidance system. % Line of argument: Parametrization P1 was selected using GO1-3, now in P2 (refining P1) we see GO4. Different guidance that changed depending on how P1 was selected.

\subsubsection{Lag Selection (Task C5)}
\label{sec:app--parameter-selection--lag-selection}

%After comparing the most dissimilar results in detail, the analyst wants to try a custom parametrization and see if the result is any different. They decided for a so far unused weight parameter (see \Fref{fig:app--usage-scenario}H) and now need to select two sets of lags. The problem is that there are a few thousand lags to choose from and analysts currently do not quantify and compare them in any way, as this also entails writing custom data mining techniques.

We support selection of a single lag set with multiple coordinated views (see \Fref{fig:app--lag-selection}). The lag size is encoded with color saturation, to make long, medium, and short lags distinguishable in all views, which is roughly how analysts reason about lag sets.

\begin{figure}
  \centering
  \includegraphics[width=\textwidth]{images/app/selection-exrates.png}
  \caption{The Lag Selection view: Lag size is encoded with color saturation. Lags are filtered to those corresponding to a temporal difference of multiple weeks in the underlying calendar. The PCP (A) further narrows them down to those with high autocorrelation . It is visible that large lags (ca. 1\,800) could also be interesting. A multivariate ACF plot (B) shows the autocorrelation of input data at brushed lags. Lags can be selected by clicking and highlighted by hovering in the ACF plot. A user-selected input time series is shown underneath (C) next to a scatterplot of the datapoints of the series at the currently highlighted lag. The right-most column (D) allows analysts to skip the interaction, and shows the current selection.}
  \label{fig:app--lag-selection}
\end{figure}

A parallel coordinates plot (PCP) displays all lags corresponding to a selected calendar granule (\Fref{fig:app--lag-selection}A), which can be configured by the user. Its dimensions are GO1–4, and values of selected lags are displayed as triangle marks next to the axes. The PCP supports common interactions such as inverting dimensions, reordering dimensions, and brushing.
% \cite{johansson2016}
It is used to reduce the parameter space to a manageable subset. This subset is then visualized in a multivariate autocorrelation function plot (MACF), so analysts can view the temporal structure of all variables (\Fref{fig:app--lag-selection}B). The MACF shows all univariate autocorrelation function plots, composited through nesting: One box contains the autocorrelations of all variables at a given lag. Autocorrelations are encoded as bars, as in the univariate version, and can be sorted by variable name or by value. The latter is the default because it shows the distribution of autocorrelation values. Hovering over a box highlights the lag, which affects the next view below it. Clicking a box adds or removes the lag from/to the selection, which is shown in the right column with the lag set visualization from \Fref{sec:app--explore}.

Underneath the MACF we display a user-selected input time series as line graph, and a scatterplot of the time series' values vs. the values lagged by the currently highlighted lag (\Fref{fig:app--lag-selection}C). This allows the analyst to find correlation patterns which are not surfaced by the MACF or the time series itself. A line on top of the time series shows the extent of the currently highlighted lag in context. % 51m vs 4y3m

These views allow the analyst to interactively explore lags. Should they exactly know what they want to select, or rather not use an interactive system because they are used to static tools, they can enter the desired lags in the input box in the right column (\Fref{fig:app--lag-selection}D) in a format similar to R's \texttt{seq} shorthand syntax and proceed.

%Our analyst, not having anything particular in mind, follows the suggestions by the system. First, they set the PCP to show weeks instead of days to reduce the amount of lines (see \Fref{fig:app--usage-scenario}I). The values of GO3 (\emph{eigenvalue difference}) seem to be quite low, and GO3's highest values (top part of the PCP axis) refer to very long lags. Short lags are usually expected to be the interesting lags, so this is somewhat odd. The analyst instead decides to use GO2 (\emph{max. autocorrelation}), filters for high values and selects the a few of the shortest lags (see \Fref{fig:app--usage-scenario}J). The analyst repeats this for months and years, and the other lag set. The analyst is then redirected back to the \textit{Explore} view, where the result will be computed in the background and selected automatically once available. Looking at the unmixing matrix comparison (see \Fref{fig:app--usage-scenario}K), the new right-most result seems to separate input variables better than the others as more white cells are visible.
